AI Urban Scientist: Multi-Agent Collaborative Automation for Urban Research

Urban research aims to understand how cities operate and evolve as complex adaptive systems. With the rapid growth of urban data and analytical methodologies, the central challenge of the field has shifted from data availability to the integration of heterogeneous data into coherent, verifiable urban knowledge through multidisciplinary approaches. Recent advances in AI, particularly the emergence of large language models (LLMs), have enabled the development of AI scientists capable of autonomous reasoning, hypothesis generation, and data-driven experimentation, demonstrating substantial potential for autonomous urban research. However, most general-purpose AI systems remain misaligned with the domain-specific knowledge, methodological conventions, and inferential standards required in urban studies. Here, we introduce the AI Urban Scientist, a knowledge-driven multi-agent framework designed to support autonomous urban research. Grounded in hypotheses, peer-review feedback, datasets, and research methodologies distilled from large-scale prior studies, the system constructs structured domain knowledge that guides LLM-based agents to automatically generate hypotheses, identify and integrate multi-source urban datasets, conduct empirical analyses and simulations, and iteratively refine analytical methods. Through this process, the framework synthesizes new insights in urban science and accelerates the urban research lifecycle.

==> 2_background.tex <==
\section*{Traditional Urban Science Research}

\subsection*{Contemporary Workflow and Challenges}
% 2.1代表性流程和面临的挑战：（云柯）

% 一个团队：提出假设，找数据-分析数据。 
% 	问题提出难：目前广被接收的Urban Science研究议题很有限（标度率等）
% 	有效假设难：依赖于专家-知识大量的经验+观察  
% -	全流程中跨学科合作难：geo science, social science, data science等 
% 	数据利用不充分：完全依赖对领域数据的了解和手工查找
% 	数据分析低效：针对特定问题，手写数据分析的代码
% 	可复用性低： 没有像ML有开源的的传统，工具少
% 	跨学科和跨领域的知识运用难：从不同学科视角和综合研究和解决城市科学问题很困难，特别是城市专业领域与人工智能/计算机领域的合作。有工具的缺真正的问题和思想，反之缺熟练掌握AI工具的人。



Contemporary urban science research still relies heavily on a linear and highly manual workflow—researchers first generate observation-driven hypotheses, then manually search for suitable datasets, and finally hand-code analytical procedures. This traditional pipeline presents several structural limitations. Problem discovery remains narrow, as widely accepted urban science questions (e.g., scaling laws) dominate the field and constrain innovation. Hypothesis formation is often weak because it depends largely on expert experience and subjective observation rather than systematic exploration. Data remain underused due to the difficulty of locating relevant sources across heterogeneous domains, and analysis is inefficient because each study requires bespoke coding and processing. Moreover, reproducibility is low, as the field lacks the open-source tooling and standardized workflows common in machine learning. These challenges are amplified by the cross-disciplinary nature of urban science: integrating perspectives from geography, sociology, public health, and data science is difficult, and collaboration between domain experts and AI/CS researchers is often hindered by asymmetric knowledge gaps. Together, these barriers limit the ability of research teams to efficiently discover problems, generate robust hypotheses, and leverage the full potential of modern urban data.



\subsection*{Current Role of AI in Urban Science}


% 近20年来，大数据对城市科学研究起到了至关重要的作用，形成了数据密集型范式下的城市科学研究之路
% 然而，AI起到的作用有限：Urban Computing是AI+大数据研究城市问题，但并没有大规模推向应用，并且对城市科学的研究帮助十分有限。
% 有些一手数据/指标难直接获取 –> 用ML model 做预测
% 实验方案与LLM进行讨论



%Cities, now home to over half of the global population, are often envisioned as engines of interaction, yet access to urban spaces and opportunities remains highly uneven~\cite{florida2017new, mallach2018divided}. 

Over the past two decades, the rise of large-scale digital traces—ranging from mobility records and social media to satellite imagery and IoT systems—has fundamentally shaped contemporary urban science, enabling a new data-intensive paradigm for understanding cities \cite{Karvonen2021NewUrbanScience}. Despite this rapid growth, the actual role of AI in advancing core urban science research remains limited.

Most existing applications fall under urban computing, where machine learning models are applied to big-data streams to address urban management tasks such as traffic prediction, energy forecasting, or crowd-flow estimation \cite{Aydogdu2022MachineLearningUrbanComputing, Chen2025MLforUrbanChallenges}. While effective in engineering contexts, these methods have not transformed how urban scientists generate hypotheses or develop theories. Their influence remains largely confined to technical prediction tasks rather than the broader scientific workflow of question discovery, hypothesis formation, and causal reasoning.

AI is also used when key urban indicators or first-hand measurements are difficult or costly to obtain—for instance, using machine learning to infer socioeconomic conditions from satellite images or to estimate mobility patterns from sparse data \cite{Wang2022UnsupervisedMLUrbanStudies}. Such predictive models help fill data gaps but do not fundamentally shift conceptual frameworks or advance the theoretical core of urban science. More recently, large language models (LLMs) have begun to enter the research process. Researchers employ LLMs for literature exploration, preliminary methodological discussions, or experiment ideation \cite{Ye2025AIinUrbanScience}. However, these uses remain informal and are not yet systematically integrated into the scientific pipeline. Early visions of how LLMs could influence urban planning and computational urbanism are emerging \cite{Zheng2025UrbanPlanningLLM}, but these developments are still at an exploratory stage.

In summary, AI currently plays a supportive rather than transformative role in urban science. It accelerates certain tasks and fills data gaps but does not yet address deeper structural challenges such as limited problem discovery, weak hypothesis formation, inefficient analytical workflows, and persistent cross-disciplinary knowledge barriers. These limitations point to the need for a new research paradigm in which AI—potentially implemented as coordinated multi-agent systems—can collaborate with human researchers to explore data, formulate questions, test hypotheses, and integrate knowledge across disciplines, ultimately enabling a more systematic and discovery-driven mode of urban science.


% \begin{figure*}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/ficture1.png}
%     \caption{\textbf{The AI urban scientist workflow.} }
%     \label{fig:framework}
% \end{figure*}



==> 3_newinsight.tex <==
\section*{Opportunities brought by AI Scientist}

\subsection*{The Emergence of AI Scientist}


% LLM agent带来的deep research 和 auto-coding 对科研范式的改变
% AI x Scientist简述：Data Scientist, Chemistry Scientist, Social scientist 

% The rapid development of large language models (LLMs) and autonomous AI agents has led to the emergence of what is increasingly described as the AI Scientist—an AI system capable of assisting, accelerating, or even autonomously executing components of the scientific research workflow \cite{Chan2023LLMScience,AI2024NatureSci}. Unlike earlier applications of machine learning that focused narrowly on prediction tasks, AI Scientist systems integrate deep reasoning, automated coding, literature understanding, and iterative experimentation, offering the potential to fundamentally reshape scientific inquiry.

% Recent advances demonstrate that LLM agents can perform deep research, including generating research questions, synthesizing theories, designing experiments, and evaluating evidence across disciplines \cite{Liu2024DeepResearch,Khoo2024AutonomousScience}. At the same time, auto-coding capabilities allow these models to translate research ideas into executable analytical pipelines, reducing the gap between conceptual reasoning and practical implementation \cite{Jain2024AutoCoding}. These combined abilities introduce a qualitatively different research paradigm—one in which AI collaborates with or augments human scientists to conduct end-to-end scientific investigations.

% The notion of the AI Scientist is already materializing across multiple domains. In data science, autonomous agents assist with data cleaning, causal reasoning, statistical modeling, and reproducible analysis workflows \cite{Narayan2024AIAgentDS}. In chemistry, AI-driven laboratory agents can autonomously propose compounds, run robotic experiments, and refine hypotheses through active learning \cite{Booth2023AIchemist}. In the social sciences, LLM-based agents are beginning to formalize theories, analyze qualitative and quantitative data, and generate structured hypotheses informed by large corpora of social information \cite{Park2023SocialAISystems}. These precedents highlight that AI Scientist systems are not isolated prototypes but emerging components of a broader transformation in scientific methodology.

% The convergence of these developments suggests that AI Scientist systems could similarly reshape urban science, a field characterized by complex systems, heterogeneous data, and cross-disciplinary theories. By combining reasoning, coding, and knowledge synthesis, AI Scientist agents offer an opportunity to address long-standing structural challenges such as limited problem discovery, inefficient analysis pipelines, and barriers to interdisciplinary collaboration. As these tools continue to mature, they may enable a more automated, exploratory, and generative mode of knowledge creation, redefining the scientific process for urban research and beyond.

The rapid advancement of large language models (LLMs) and autonomous AI agents has given rise to the concept of the AI Scientist—an AI system capable of assisting, accelerating, or even autonomously executing core components of the scientific workflow \cite{Chan2023LLMScience,AI2024NatureSci}. Unlike earlier machine-learning applications focused mainly on prediction, AI Scientist systems integrate deep reasoning, automated coding, literature understanding, and iterative experimentation. Recent work demonstrates that LLM agents can generate research questions, synthesize theories, design experiments, and evaluate evidence \cite{Liu2024DeepResearch,Khoo2024AutonomousScience}, while auto-coding capabilities translate ideas into executable analytical pipelines \cite{Jain2024AutoCoding}. These advances have already begun reshaping fields such as data science \cite{Narayan2024AIAgentDS}, chemistry \cite{Booth2023AIchemist}, and the social sciences \cite{Park2023SocialAISystems}. Together, they suggest that AI Scientist systems could similarly transform urban science, enabling more automated, exploratory, and generative knowledge creation across its complex, data-rich research landscape.

\subsection*{How Can AI Scientist Help with Urban Science}


% - 加快ideation（问题提出，假设提出）
% - 更高效的引入跨学科的知识
% - 更全面的data search
% - 自动化的实验方案生成和数据分析
% - 提供可复用的工具、加速社区建设



The AI Scientist framework offers transformative opportunities for urban science by reshaping each step of the scientific workflow—from problem discovery to hypothesis building, data acquisition, analysis, and publication. As depicted in Figure~\ref{fig:1}, AI agents can operate as research collaborators capable of synthesizing knowledge, automating analysis, and bridging disciplinary divides \cite{Chan2023LLMScience,AI2024NatureSci}. Below, we outline several key ways in which AI Scientist systems can advance urban science.

\begin{itemize}

 \item \textit{Accelerating Ideation}. Problem Discovery and Hypothesis Formation.
Urban science has long suffered from a narrow band of canonical research problems and a heavy reliance on expert intuition. AI Scientist agents can explore large corpora of literature, extract underexplored topics, generate novel research directions, and synthesize interdisciplinary theories \cite{Liu2024DeepResearch}. These systems can identify emerging urban challenges—ranging from environmental risks to socio-spatial inequalities—and propose testable hypotheses at a pace and breadth far beyond human capability. This capability is particularly valuable in urban settings, where questions often span geography, sociology, economics, environmental science, and engineering.

 \item \textit{Enhancing Interdisciplinary Knowledge Integration.}
Urban phenomena are inherently cross-disciplinary, yet integrating theories from disparate fields is one of the most persistent bottlenecks in urban research. LLM-based AI Scientist systems excel at retrieving, summarizing, and reconciling knowledge across the social sciences, environmental sciences, public health, and computational modeling \cite{Park2023SocialAISystems}. By contextualizing a hypothesis within multiple disciplines, AI Scientist supports more comprehensive reasoning and fosters intellectually diverse urban inquiry.

 \item \textit{Comprehensive and Automated Data Search.}
Identifying suitable datasets is often one of the most time-consuming steps in urban science. AI agents can perform broad data discovery across open data portals, scientific archives, satellite sources, and sensor datasets. Recent developments in LLM-guided dataset retrieval \cite{Narayan2024AIAgentDS} allow the AI Scientist to match hypotheses with relevant data sources, assess data fitness, and even suggest complementary datasets to enrich analysis. This greatly reduces the manual burden and expands the scope of empirical studies.

 \item \textit{Automated Experimental Design and Data Analysis.}
Through auto-coding and LLM-to-code translation capabilities \cite{Jain2024AutoCoding}, AI Scientist systems can automatically generate analytical pipelines—ranging from causal inference models and spatial econometrics to simulation workflows and machine learning pipelines for environmental prediction. This not only accelerates research execution but also increases reproducibility by producing self-documented code, structured outputs, and standardized evaluation procedures. In urban science—where data can be noisy, high-dimensional, or incomplete—AI Scientist systems can also propose alternative analyses or robustness checks autonomously.

 \item \textit{Providing Reusable Tools and Accelerating Community Building.}
A major limitation of current urban science is the lack of shared computational tools and standardized workflows. AI Scientist agents can help create modular, reusable codebases, automated templates for data processing, and shared analytical components that reduce redundancy across research groups. This mirrors the open-source tradition of machine learning but brings it into the urban science domain, fostering community-building and improving reproducibility across studies \cite{Khoo2024AutonomousScience}.

    
\end{itemize}

In summary, AI Scientist systems offer a powerful means to overcome the structural challenges of contemporary urban science. By accelerating ideation, enabling interdisciplinary synthesis, enhancing data accessibility, automating analyses, and fostering tool-sharing, AI Scientist has the potential to transition the field from a manual, expert-driven paradigm toward a more systematic, scalable, and discovery-oriented mode of scientific inquiry.
